On Upper Bounds on the Church-Rosser Theorem

The Church-Rosser theorem in the type-free lambda-calculus is well investigated both for beta-equality and beta-reduction. We provide a new proof of the theorem for beta-equality with no use of parallel reductions, but simply with Takahashi's translation (Gross-Knuth strategy). Based on this, upper bounds for reduction sequences on the theorem are obtained as the fourth level of the Grzegorczyk hierarchy.

==> eptcsdata.tex <==
\providecommand{\firstpage}{16}
\providecommand{\publicationstatus}{H. Cirstea, S. Escobar (Eds.): Third International Workshop on Rewriting\\ 
Techniques for Program Transformations and Evaluation (WPTE'16).
\\
EPTCS 235, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.235.2}{10.4204/EPTCS.235.2}}
\pdfoutput=1

